Anytime Replanning of Robot Coverage Paths for Partially Unknown Environments

In this paper, we propose a method to replan coverage paths for a robot operating in an environment with initially unknown static obstacles. Existing coverage approaches reduce coverage time by covering along the minimum number of coverage lines (straight-line paths). However, recomputing such paths online can be computationally expensive resulting in robot stoppages that increase coverage time. A naive alternative is greedy detour replanning, i.e., replanning with minimum deviation from the initial path, which is efficient to compute but may result in unnecessary detours. In this work, we propose an anytime coverage replanning approach named OARP-Replan that performs near-optimal replans to an interrupted coverage path within a given time budget. We do this by solving linear relaxations of integer linear programs (ILPs) to identify sections of the interrupted path that can be optimally replanned within the time budget. We validate OARP-Replan in simulation and perform comparisons against a greedy detour replanner and other state-of-the-art coverage planners. We also demonstrate OARP-Replan in experiments using an industrial-level autonomous robot.

==> Sections/algorithm_analysis.tex <==
\subsection{Algorithm Analysis}

We now analyze our algorithm and describe the purpose of the two stages. For this, we first clarify the main problem we are aiming to solve. Let $\mathcal{P}$ be the feasible solution space for the rank replanning problem. More specifically, $\mathcal{P}$ represents all combinations of grid cell orientations and their corresponding endpoints. For a solution $\boldsymbol{x} \in \mathcal{P}$, let $m_{\text{new}}(\boldsymbol{x})$ be the number of new ranks, and $m_{\text{old}}(\boldsymbol{x})$ be the number of old ranks retained from the initial coverage path. The number of total ranks $m(\boldsymbol{x})$ is computed as follows:
\begin{align}
    m(\boldsymbol{x}) = m_{\text{new}}(\boldsymbol{x}) + m_{\text{old}}(\boldsymbol{x}).
    \label{eq:m_total_sum}
\end{align}

Now, consider obtaining the true optimal coverage path for the remainder of the environment. We get this path by solving the following problem:
\begin{align*}
    \text{\textbf{OPT}:} \quad \min_{\boldsymbol{x}} &\quad m(\boldsymbol{x})\\
    \textrm{s.t.} &\quad \boldsymbol{x} \in \mathcal{P}.
    % &\quad m_{\text{new}}(\boldsymbol{x}) \leq \Bar{m}.
\end{align*}
Let $\boldsymbol{x}_\text{O}^*$ be the optimizer of this problem. We now consider the proposed rank replanning problem with the budget constraint, which we obtain by adding a constraint to \textbf{OPT} as follows:
\begin{align*}
    \text{\textbf{REPLAN}:} \quad \min_{\boldsymbol{x}} &\quad m(\boldsymbol{x})\\
    \textrm{s.t.} &\quad \boldsymbol{x} \in \mathcal{P}, \\
    &\quad m_{\text{new}}(\boldsymbol{x}) \leq \Bar{m}.
\end{align*}
While the budget constraint allows us to replan a tour of the ranks without stoppage, it affects the quality of the path in terms of the number of ranks. Therefore, it is useful to obtain an approximation factor for the number of ranks obtained from solving \textbf{REPLAN}. 

Let $\boldsymbol{x}_\text{R}$ be a feasible solution for \textbf{REPLAN}. We now obtain a performance guarantee for this solution with respect to the $\boldsymbol{x}_\text{O}^*$. For this, we require one other component. Let $m_\text{initial}$ be the number of ranks in the initial coverage path. From its definition, we have the following relation with the number of old ranks in the replanned solution:
\begin{align}
    m_{\text{old}}(\boldsymbol{x}) \leq m_\text{initial}.
    \label{eq:initial_ranks_bound}
\end{align}

\begin{theorem*}
    Let $\boldsymbol{x}_\text{R}$ be a feasible solution for \textbf{REPLAN} and $\boldsymbol{x}_\text{O}^*$ be the optimizer of \textbf{OPT}. Given that $m_\text{initial}$ is the number of ranks in the initial path and $\Bar{m}$ is the budget for the number of new ranks, $m(\boldsymbol{x}_\text{R})$ follows:
    \begin{align*}
        m(\boldsymbol{x}_\text{R}) \leq (1 + \frac{m_\text{initial}}{\Bar{m}}) m(\boldsymbol{x}_\text{O}^*)
    \end{align*}
\end{theorem*}
\begin{proof}
    We start by assuming that $\boldsymbol{x}_\text{O}^*$ is not a feasible solution for \textbf{REPLAN}. Otherwise, solving \textbf{REPLAN} gives us an optimizer to \textbf{OPT} with no approximation. With this assumption, we have the following inequality:
    \begin{align*}
        \Bar{m} \leq m_{\text{new}}(\boldsymbol{x}_\text{O}^*).
    \end{align*}
    Now, from Eq. (\ref{eq:m_total_sum}), we have the following breakdown of $m(\boldsymbol{x}_\text{R})$:
    \begin{align*}
        m(\boldsymbol{x}_\text{R}) = m_{\text{new}}(\boldsymbol{x}_\text{R}) + m_{\text{old}}(\boldsymbol{x}_\text{R}).
    \end{align*}
    However, since $\boldsymbol{x}_\text{R}$ is a feasible solution of \textbf{REPLAN}, we have the following bound for $m_{\text{new}}(\boldsymbol{x}_\text{R})$:
    \begin{align*}
        m_{\text{new}}(\boldsymbol{x}_\text{R}) \leq \Bar{m}.
    \end{align*}
    Using this and Eq. (\ref{eq:initial_ranks_bound}), we have the following bound for $m(\boldsymbol{x}_\text{R})$:
    \begin{align*}
        m(\boldsymbol{x}_\text{R}) &\leq \Bar{m} + m_\text{initial} \\
        &\leq (1 + \frac{m_\text{initial}}{\Bar{m}})\Bar{m} \\
        &\leq (1 + \frac{m_\text{initial}}{\Bar{m}})m_{\text{new}}(\boldsymbol{x}_\text{O}^*).
    \end{align*}
    However, from Eq. (\ref{eq:m_total_sum}), we have that $m_{\text{new}}(\boldsymbol{x}_\text{O}^*) \leq m(\boldsymbol{x}_\text{O}^*)$. Therefore, we obtain the following performance guarantee for \textbf{REPLAN}:
    \begin{align}
        m(\boldsymbol{x}_\text{R}) &\leq (1 + \frac{m_\text{initial}}{\Bar{m}})m(\boldsymbol{x}_\text{O}^*)
    \end{align}
\end{proof}

We now analyze the two-stage algorithm and describe the purpose of the two stages. For this, we first clarify the main problem we are aiming to solve. The \textbf{S1} and \textbf{S2} problems can be written similarly to \textbf{REPLAN} by replacing $m_{\text{new}}(\boldsymbol{x})$ with the corresponding bounds. First, we establish the purpose of the \textbf{S1} problem as a means to find the optimal solution of \textbf{REPLAN}.

\begin{theorem*}
Let $\boldsymbol{x_1^*}$ be an optimizer of \textbf{S1}. If $m_{\text{new}}(\boldsymbol{x_1^*}) \leq \Bar{m}$, then $\boldsymbol{x_1^*}$ is an optimizer of \textbf{REPLAN}.
\end{theorem*}
\begin{proof}
    Let $\boldsymbol{x_R^*}$ be an optimizer of \textbf{REPLAN}. Since $m_{\text{new}}(\boldsymbol{x_1^*}) \leq \Bar{m}$, $\boldsymbol{x_1^*}$ is a feasible solution of \textbf{REPLAN}. Therefore, we have the following.
    \begin{align*}
        m(\boldsymbol{x_R^*}) \leq m(\boldsymbol{x_1^*}).
    \end{align*}
    However, from the definition of \textbf{REPLAN} and Lemma \ref{lem:endpoints}, we get the following relation for $\boldsymbol{x_R^*}$:
    \begin{align*}
        \alpha(\boldsymbol{x_R^*})/2 \leq m_{\text{new}}(\boldsymbol{x_R^*}) \leq \Bar{m}.
    \end{align*}
    This indicates that $\boldsymbol{x_R^*}$ is a feasible solution to \textbf{S1}, and therefore, we have the following:
    \begin{align*}
        m(\boldsymbol{x_1^*}) \leq m(\boldsymbol{x_R^*}).
    \end{align*}
    The above is true only if $m(\boldsymbol{x_1^*}) = m(\boldsymbol{x_R^*})$, which indicates that $\boldsymbol{x_1^*}$ is an optimizer for \textbf{REPLAN}, thereby proving our lemma.
\end{proof}
From this lemma, we observe that if we obtain $\boldsymbol{x_1^*}$ and verify that $m_{\text{new}}(\boldsymbol{x_1^*}) \leq \Bar{m}$, we have obtained the optimizer for the rank replanning problem. Moreover, the addition of the added endpoint constraint eliminates solutions with really large changes to the initial ranks, as opposed to not including it. Note that \textbf{REPLAN} may not necessarily have a unique optimizer. In the case that it does, we can extend the above argument to indicate that $\boldsymbol{x_1^*} = \boldsymbol{x_R^*}$. 

However, \textbf{S1} may return a solution where $m_{\text{new}}(\boldsymbol{x_1^*}) > \Bar{m}$. In this case, we solve \textbf{S2} which, if feasible, guarantees a solution that respects the budget constraint. The solution may however be a sub-optimal solution. Another thing to note is that there may be instances where \textbf{S2} may not be feasible while \textbf{REPLAN} may still have a feasible solution. In the next section, we deal with this case by planning greedy detour paths to reduce the replanning problem size and give us additional time to replan the remainder of the path, i.e. a larger $\Bar{m}$. From our experiments, however, we encountered very few instances where \textbf{S2} does not return a feasible solution.

%%% Opt factor might be incorrect
%% If m(x) <= m_new(x), then S2 would have to return the same solution as Replan if feasible.

%% Can we actually use Lagrangian to analyze optimality?

% To obtain an optimality factor, we analyze the worst-case scenario where the budget constraint directly influences the objective value. Consider the case where none of the ranks from the previous path can be retained as they are all interrupted by obstacles, i.e. $m_{\text{new}}(\boldsymbol{x}) = m(\boldsymbol{x})$. We assume that no rank has been fully blocked by an obstacle to the extent that the rank can simply be removed from the path. For this case, we obtain the following optimality factor for the \textbf{S2} approach:

% \begin{theorem*}
%     Consider the above worst-case scenario where $m_{\text{new}}(\boldsymbol{x}) = m(\boldsymbol{x})$ and let $\boldsymbol{x_R^*}$ be an optimizer of \textbf{REPLAN}. The optimizer of \textbf{S2}, namely $\boldsymbol{x_2^*}$, follows:
%     \begin{align*}
%         m(\boldsymbol{x_2^*}) \leq 3 m(\boldsymbol{x_R^*})
%     \end{align*}
% \label{thm:approx-factor}
% \end{theorem*}

% Before we prove the above theorem, we establish the following relation between $\alpha(\boldsymbol{x})$ and $\beta(\boldsymbol{x})$ in this worst-case scenario. We will use this relation in our proof of Theorem \ref{thm:approx-factor}.

% \begin{lemma}
%     Given the worst-case scenario where $m_{\text{new}}(\boldsymbol{x}) = m(\boldsymbol{x})$, $\beta(\boldsymbol{x}) \leq \alpha(\boldsymbol{x})$.
%     \label{lem:beta-alpha-rel}
% \end{lemma}
% \begin{proof}
%     Since every rank from the previous path is interrupted, every new rank must have at least one added endpoint. This includes ranks that have merged into larger ranks and ranks that have been extended. Therefore, for each rank endpoint that has been extended, at least one rank endpoint is added. Therefore, we have $\beta(\boldsymbol{x}) \leq \alpha(\boldsymbol{x})$, proving our lemma.
% \end{proof}

% We now prove Theorem \ref{thm:approx-factor}.

% \begin{proof}[Proof of Theorem \ref{thm:approx-factor}]
% We start by considering the case where $\alpha(\boldsymbol{x_R^*}) + \beta(\boldsymbol{x_R^*})/2 \leq \Bar{m}$. In this case, $\boldsymbol{x_R^*}$ is clearly a feasible solution for \textbf{S2} and that $m(\boldsymbol{x_R^*}) = m(\boldsymbol{x_2^*})$, indicating that $\boldsymbol{x_2^*}$ is an optimizer of \textbf{REPLAN}. While this shows that \textbf{S2} can obtain an optimal solution for \textbf{REPLAN}, we cannot verify this as we have no knowledge of what $\boldsymbol{x_R^*}$ is.

% Therefore, we assume the worst case where $\boldsymbol{x_R^*}$ is not a feasible solution for \textbf{S2}. Therefore, we have:
% \begin{align*}
%      \Bar{m} \leq \alpha(\boldsymbol{x_R^*}) + \beta(\boldsymbol{x_R^*})/2.
% \end{align*}
% From Lemmas \ref{lem:endpoints} and \ref{lem:beta-alpha-rel}, we have the following relation:
% \begin{align}
%      \nonumber \Bar{m} \leq \alpha(\boldsymbol{x_R^*}) + \beta(\boldsymbol{x_R^*})/2 \leq 3 \alpha(\boldsymbol{x_R^*}) / 2 \\ 
%      \Bar{m} \leq 3 m_{\text{new}}(\boldsymbol{x_R^*}) = 3 m(\boldsymbol{x_R^*}).
% \end{align}
% However, from the definition of \textbf{S2} we have $m(\boldsymbol{x_2^*}) =  m_{\text{new}}(\boldsymbol{x_2^*}) \leq \Bar{m}$. Using this, we get the following relation between $m(\boldsymbol{x_2^*})$ and $m(\boldsymbol{x_R^*})$:
% \begin{align*}
%     m(\boldsymbol{x_2^*}) \leq 3 m(\boldsymbol{x_R^*}),
% \end{align*}
% thereby proving our lemma.
% \end{proof}

